When Does Differentially Private Learning Not Suffer in High Dimensions?

Large pretrained models can be privately fine-tuned to achieve performance approaching that of non-private models. A common theme in these results is the surprising observation that high-dimensional models can achieve favorable privacy-utility trade-offs. This seemingly contradicts known results on the model-size dependence of differentially private convex learning and raises the following research question: When does the performance of differentially private learning not degrade with increasing model size? We identify that the magnitudes of gradients projected onto subspaces is a key factor that determines performance. To precisely characterize this for private convex learning, we introduce a condition on the objective that we term \emph{restricted Lipschitz continuity} and derive improved bounds for the excess empirical and population risks that are dimension-independent under additional conditions. We empirically show that in private fine-tuning of large language models, gradients obtained during fine-tuning are mostly controlled by a few principal components. This behavior is similar to conditions under which we obtain dimension-independent bounds in convex settings. Our theoretical and empirical results together provide a possible explanation for recent successes in large-scale private fine-tuning. Code to reproduce our results can be found at \url{https://github.com/lxuechen/private-transformers/tree/main/examples/classification/spectral_analysis}.

==> intro.tex <==
\section{Introduction}

Recent works have shown that large publicly pretrained models can be differentially privately fine-tuned on small downstream datasets with performance approaching those attained by non-private models. 
In particular, past works showed that pretrained BERT~\cite{devlin2018bert} and GPT-2~\cite{radford2018improving,radford2019language} models can be fine-tuned to perform well for text classification and generation under a privacy budget of $\epsilon \in [2, 6]$~\cite{li2021large,yu2021differentially}. 
More recently, it was shown that pretrained ResNets~\cite{he2016deep} and vision-Transformers~\cite{dosovitskiy2020image} can be fine-tuned to perform well for ImageNet classification under single digit privacy budgets~\cite{de2022unlocking,mehta2022large}. 

One key ingredient in these successes has been the use of large pretrained models with millions to billions of parameters. 
These works generally highlighted the importance of two phenomena: (i) large pretrained models tend to experience good privacy-utility trade-offs when fine-tuned, and (ii) the trade-off improves with the use of larger models.
While the power of scale and pretraining has been demonstrated numerous times in non-private deep learning, one common wisdom in private learning had been that large models tend not to perform well.
This intuition was based on results in differentially private convex optimization, which predicted that errors would scale proportionally with the dimension of the learning problem. 

Consider the problem of differentially private convex \emph{empirical risk minimization} (ERM) as an example.
In this problem, we are given a dataset of $n$ examples $\cD = \{s_j\}_{j=1}^n \in \mathcal{S}^{n}$, a convex body $\cK\subset \R^{d}$, and the goal is to perform the optimization
\eqn{
	\text{minimize}_{x\in \cK} F(x; \cD) = \frac{1}{n} \sum_{j=1}^n f(x; s_j)
}
subject to differential privacy, 
where $f(\cdot;s)$ is some convex loss function over $\cK$ for all $s\in \mathcal{S}$. 
Past works have studied this problem and presented matching upper and lower bounds that are dimension-dependent under the usual Lipschitz assumptions on the objective~\cite{bassily2014private,chaudhuri2011differentially}.
These dimension-dependent results suggest that the performance of differentially private convex ERM inevitably degrades with increasing problem dimension --- for the worst case functions within the prescribed class of convex losses. 

To reconcile the conflict between the dimension-dependent lower bounds for private convex learning and the empirical success of large-scale private fine-tuning, we study the following question both theoretically and empirically:
\begin{quote}
	\centering
	\emph{When does the performance of differentially private learning (via DP-SGD) not degrade with increasing problem dimension?}
\end{quote}


On the theoretical front, we identify that the standard dependence on the dimension of the ambient space can be replaced by the magnitudes of gradients projected onto subspaces of varying dimensions.
We formalize this in a condition that we call \textit{restricted Lipschitz continuity} and derive refined bounds for the excess empirical risks for DP-ERM and population risks for DP-SGD when loss functions obey this condition. 
We show that when the restricted Lipschitz coefficients decay rapidly, both the excess empirical and population risks become dimension-independent.

These theoretical results shed light on the recent success of large-scale private fine-tuning of language models.
We empirically show that the gradients of language models during fine-tuning are mostly controlled by a few principal components --- a behavior that is similar to conditions under which we obtain dimension-independent bounds for private convex ERM. 
This provides a possible explanation for the observation that densely fine-tuning (with DP-SGD) need not necessarily have much worse performance than sparsely fine-tuning~\cite{li2021large}. Moreover, it suggests that DP-SGD can be adaptive to problems that are effectively low-dimensional (as characterized by restricted Lipschitz continuity) without explicit algorithmic intervention.
We summarize our contributions below.
\begin{itemize}[leftmargin=7mm]
\setlength\itemsep{0.1em}
	\item [(1)] We introduce a condition on the objective function that we term restricted Lipschitz continuity.
		This condition generalizes the usual Lipschitz continuity notion and gives rise to refined analyses when magnitudes of gradients projected onto diminishing subspaces decay rapidly.
	\item [(2)] Under restricted Lipschitz continuity, we present refined bounds on the excess empirical and population risks for DP-SGD when optimizing convex objectives. These bounds generalize previous dimension-independent results~\cite{song2021evading} and are broadly applicable to cases where gradients are full rank but most coordinates only marginally influence the objective.
	\item [(3)] We study an additional setting where DP-SGD is performed in a randomly sampled subspace of possibly much smaller dimension and theoretically show that dimension-independent excess risk bounds can be obtained under restricted Lipschitz continuity with rapidly decaying coefficients.
	\item [(4)] Our theory sheds light on recent successes of private fine-tuning of language models.
		We show that gradients obtained through fine-tuning mostly lie in a subspace spanned by a few principal components --- a behavior similar to when optimizing a restricted Lipschitz continuous loss with decaying coefficients.
		This provides a possible explanation for recent successes in large-scale private fine-tuning.
\end{itemize}


==> intro_v2.tex <==
\section{Introduction}

Recent works have shown that large publicly pretrained models can be differentially privately fine-tuned on small downstream datasets with performance approaching those attained by non-private models. 
In particular, past works showed that pretrained BERT~\cite{devlin2018bert} and GPT-2~\cite{radford2018improving,radford2019language} models can be fine-tuned to perform well for text classification and generation under a privacy budget of $\epsilon \in [2, 6]$~\cite{li2021large,yu2021differentially}. 
More recently, it was shown that pretrained ResNets~\cite{he2016deep} and vision-Transformers~\cite{dosovitskiy2020image} can be fine-tuned to perform well for ImageNet classification under single digit privacy budgets~\cite{de2022unlocking,mehta2022large}. 

One key ingredient in these successes has been the use of large pretrained models with millions to billions of parameters. 
These works generally highlighted the importance of two phenomena: (i) large pretrained models tend to experience good privacy-utility trade-offs when fine-tuned, and (ii) the trade-off improves with the increase in the size of the pretrained model.
While the power of scale and pretraining have been demonstrated numerous times in non-private deep learning~\cite{kaplan2020scaling}, one common wisdom in private learning had been that large models tend not to perform well.
This intuition was based on (a) results in differentially private convex optimization, most of which predicted that errors would scale proportionally with the dimension of the learning problem, and (b) empirical observations that the noise injected to ensure privacy tends to exceed the gradient in magnitude for large models~\cite{yu2021not,gautum14}. 

For instance, consider the problem of differentially private convex \emph{empirical risk minimization} (ERM).
Here, we are given a dataset of $n$ examples $\cD = \{s_j\}_{j=1}^n \in \mathcal{S}^{n}$, a convex set $\cK \subseteq \R^{d}$ (not necessarily bounded), and the goal is to perform the optimization
\eqn{
	\text{minimize}_{x\in \cK} F(x; \cD) = \frac{1}{n} \sum_{j=1}^n f(x; s_j)
}
subject to differential privacy, 
where $f(\cdot;s)$ is convex over $\cK$ for all $s\in \mathcal{S}$. 
For bounded $\cK$, past works presented matching upper and lower bounds that are dimension-dependent under the usual Lipschitz assumption on the objective~\cite{bassily2014private,chaudhuri2011differentially}.
These results seem to suggest that the performance of differentially private ERM algorithms inevitably degrades with increasing problem size in the worst case, and present a seeming discrepancy between recent empirical results on large-scale fine-tuning.\footnote{We judiciously choose to describe the discrepancy as ``seeming'', since the refined analysis presented in the current work suggests that the discrepancy is likely non-existent.}

To better understand the relation between problem size and the performance of differentially private learning, we study the following question both theoretically and empirically:
\begin{quote}
	\centering
	\emph{When does the performance of differentially private stochastic gradient descent (DP-SGD) not degrade with increasing problem dimension?}
\end{quote}

On the theoretical front, we show that DP-SGD can result in dimension-independent error bounds even when gradients span the entire ambient space for unconstrained optimization problems.
We identify that the standard dependence on the dimension of the ambient space can be replaced by the magnitudes of gradients projected onto subspaces of varying dimensions.
We formalize this in a condition that we call \textit{restricted Lipschitz continuity} and derive refined bounds for the excess empirical and population risks for DP-SGD when loss functions obey this condition. 
We show that when the restricted Lipschitz coefficients decay rapidly, both the excess empirical and population risks become dimension-independent.
This extends a previous work which derived rank-dependent bounds for learning generalized linear models in an unconstrained space~\cite{song2021evading}. 

Our theoretical results shed light on the recent success of large-scale private fine-tuning.
We empirically show that gradients of language models during fine-tuning are mostly controlled by a few principal components --- a behavior that is similar to conditions under which we obtain dimension-independent bounds for private convex ERM. 
This provides a possible explanation for the observation that densely fine-tuning with DP-SGD need not necessarily experience much worse performance than sparsely fine-tuning~\cite{li2021large}. Moreover, it suggests that DP-SGD can be adaptive to problems that are effectively low-dimensional (as characterized by restricted Lipschitz continuity) without explicit algorithmic intervention.
We summarize our contributions below.
\begin{itemize}[leftmargin=7mm]
\setlength\itemsep{0.1em}
	\item [(1)] We introduce a condition on the objective function that we term restricted Lipschitz continuity.
		This condition generalizes the usual Lipschitz continuity notion and gives rise to refined analyses when magnitudes of gradients projected onto diminishing subspaces decay rapidly.
	\item [(2)] Under restricted Lipschitz continuity, we present refined bounds on the excess empirical and population risks for DP-SGD when optimizing convex objectives. These bounds generalize previous dimension-independent results~\cite{song2021evading} and are broadly applicable to cases where gradients are full rank but most coordinates only marginally influence the objective.
	\item [(3)] As a byproduct of the new techniques, we study an additional setting where DP-SGD is ran in a random subspace of possibly much smaller dimension. We show that dimension-independent excess risk bounds can be obtained under the same decaying coefficients condition on the objective. This provides a likely explanation of the empirical success of sparse fine-tuning approaches~\cite{hu2021lora,houlsby2019parameter,karimi2021compacter}.
	\item [(4)] Our theory sheds light on recent successes of large-scale private fine-tuning of language models.
		We show that gradients obtained through fine-tuning mostly lie in a subspace spanned by a few principal components --- a behavior similar to when optimizing a restricted Lipschitz continuous loss with decaying coefficients.
		These empirical results provide a possible explanation for the recent success in large-scale private fine-tuning.
\end{itemize}


==> no_weitht_decay.tex <==
\section{No weight decay}
Suppose we do not add regularizer, i.e. $\alpha=0$ in the SGD. We show how to get similar (dimension-independent) bound.

    
    
    

\begin{lemma}
    \label{lem:radius_no_weightdecay}
    Suppose Assumption~\ref{assm:G_k} holds.
    We know
\begin{align*}
        \E\|x^{(t)}-x^{*}\|_2^{2}\leq D^2+ t\eta^2G_0^2(1+r\sigma^2).
    \end{align*}
\end{lemma}

\begin{proof}
    Let $z^{(t)}=x^{(t)}-x^*$.
    Note that 
    \begin{align*}
        z^{(t+1)}=z^{(t)}-\eta(\nabla f_{j}(x^{(t)})+G_{0}\cdot\zeta ),
    \end{align*}
    where $\zeta\sim \cN(0,\sigma^{2}I_d)$ is the isotropic Gaussian noise drawn in $(t+1)$th step. 
    For simplicity, we use $\Tnabla f_j(x^{(t)})$ to denote the noisy subgradient $\nabla f_{j}(x^{(t)})+G_{0}\cdot\zeta$.
    Hence, we have
    \begin{align*}
        \|z^{(t+1)}\|_2^2=& ~ \|z^{(t)}\|_2^2-2\eta( z^{(t)})^\top \Tnabla f_j(x^{(t)})+\eta^2\|\Tnabla f_j(x^{(t)})\|_2^2.
    \end{align*}
    
    Taking expectation over the random sample $f_j$ and random Gaussian noise $\zeta$, we have
    \begin{align*}
    \E\|z^{(t+1)}\|_{2}^{2}= &\E\|z^{(t)}\|_{2}^{2}-2\eta\E\Big((z^{(t)})^{\top}(\nabla F(x^{(t)}))\Big)  +\eta^{2}\E\|\Tnabla f_j(x^{(t)})\|_{2}^{2}.
    \end{align*}
    Noting that $\langle z^{(t)},\nabla F(x^{(t)})\rangle\ge 0$, one has
    \begin{align*}
        \E\|z^{(t+1)}\|_{2}^{2}\leq  &\E\|z^{(t)}\|_{2}^{2}+\eta^{2}\E\|\Tnabla f_j(x^{(t)})\|_{2}^{2}\\
        \leq & \E\|z^{(t)}\|_{2}^{2}+\eta^2 G_0^2(1+d\sigma^2).
    \end{align*}
    The assumption that $\|z^{(0)}\|_2\le D$ and computing by induction complete the proof.
\end{proof}

\begin{lemma}
    \label{lm:utility_DPSGD_noweight_decay}
    Let $\delta \in (0, \frac{1}{2}]$, and $\epsilon \in (0, 10]$.
    Under Assumption~\ref{assm:G_k}, let $x^{(0)}$ be the initial iterate and $x^{*} \in \R^d$ be such that $\|x^{(0)}-x^{*}\|_2\le D$.
    For all $k \in [d]$,
    setting $T=\Theta(n^2 + d \log^2 d)$,
     $\sigma=\Theta \bracks{ \frac{\sqrt{T\log(1/\delta)}}{n\epsilon} }$, and $\eta=\sqrt{\frac{D^{2}}{T\cdot G_{0}^{2}\cdot k\sigma^{2}}}$, we have
    \begin{align*}
        \E[ F(\ox)-F(x^*)]\lesssim \frac{G_0D\sqrt{k\log(1/\delta)}}{\epsilon n}+G_kD\sqrt{d/k}.
    \end{align*}
    where $\overline{x}$ is the output of DP-SGD, and the expectation is under the randomness of DP-SGD.
\end{lemma}

\begin{proof}
    We define the following set of subspaces:
    \begin{itemize}
    \item $U_{0}=\text{range}(P_{k})$.
    \item Let $U_S\bot U_0$.
    \end{itemize}
    We denote $P_0$ and $P_S$ the corresponding orthogonal projection matrices.
    Let $j \in [n]$ be the (uniformly random) index sampled in iteration $t$ of DP-SGD.
    By convexity of the individual loss $f_j$,
    \begin{align*}
        f_{j}(x^{(t)})-f_{j}(x^{*})\leq\nabla f_{j}(x^{(t)})^{\top}(x^{(t)}-x^{*}).
    \end{align*}
    By construction, $\R^d$ is the orthogonal direct sum of the subspaces $\{U_j\}_{j=0}^S$, and thus any vector $v\in \R^d$ can be rewritten as the sum $\sum_{i=0}^S Q_i v $.
    We thus split the right hand side of the above as follows
    \begin{align}
    f_{j}(x^{(t)})-f_{j}(x^{*}) & \leq \lp Q_{0}\nabla f_{j}(x^{(t)})+Q_{s}\nabla f_{j}(x^{(t)})\rp^{\top}(x^{(t)}-x^{*}).\label{eq:mirror_two_term_noweightdecay}
    \end{align}

    We can bound $ \lp Q_{0}\nabla f_{j}(x^{(t)})\rp ^\top (x^{(t)}-x^*)$ similarly to the analysis in \cite{song2021evading}.
    In particular, we have
    \begin{align*}
        \E[\|Q_0(x^{(t+1)}-x^*)\|_2^2]\leq \E[\|Q_0(x^{(t)}-x^*)\|_2^2 ]-2\eta \E[\langle F(x^{(t)}), Q_0(x^{(t)})-x^*\rangle]+\eta^2G_0^2(1+k\sigma^2).
    \end{align*}

    Hence we have
    \begin{align*}
        \E[\langle F(x^{(t)}), Q_0(x^{(t)})-x^*\rangle]\leq \frac{1}{2\eta}(\E[\|Q_0(x^{(t)}-x^*)\|_2^2 ]-\E[\|Q_0(x^{(t+1)}-x^*)\|_2^2])+\frac{\eta}{2}(G_0^2+k\sigma^2).
    \end{align*}

    As for the other term, by Lemma~\ref{lem:radius_no_weightdecay}, we have
    \begin{align*}
        \E\left[\lp Q_{s}\nabla f_{j}(x^{(t)})\rp^{\top}(x^{(t)}-x^{*})\right]\leq&~ G_{k}\|Q_s (x^{(t)}-x^*)\|_2\\
        \leq & ~G_{k}\sqrt{D^2+t\eta^2G_0^2(1+d\sigma^2)}\\
        \leq & ~G_{k}(D+\sqrt{t(1+d\sigma^2)}\eta G_0).
    \end{align*}
    Summing up for all $t\in[T]$, we have
    \begin{align*}
        \E[ F(\ox)-F(x^*)]\leq \frac{D^2}{2\eta T}+\frac{\eta}{2}G_0^2(1+k\sigma^2)+G_kD+\eta G_kG_0\sqrt{(1+d\sigma^2)T}.
    \end{align*}
    Taking back the parameters, we have
    \begin{align*}
        \E[ F(\ox)-F(x^*)]\lesssim \frac{G_0D\sqrt{k\log(1/\delta)}}{\epsilon n}+G_kD+G_kD\sqrt{d/k}.
    \end{align*}
\end{proof}


    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    


==> subspace_extension.tex <==
\section{Dimension-Independence via Optimizing in Random Subspace}
In previous sections, we showed that dimension-independent excess risk bounds can be obtained if gradients are in a near low-dimensional subspace even when we optimize with respect to all problem parameters.
We now show that dimension-independence is also achievable if we optimized in a \emph{randomly} chosen subspace --- possibly of much smaller dimension than that of the ambient space. 
This section is motivated by recent empirical studies of sparse fine-tuning and the \emph{intrinsic dimension} of language models~\cite{aghajanyan2020intrinsic}.
Before presenting the result, we include the pseudocode of the method in Algorithm~\ref{alg:opt_random_subspace} for completeness. 
\begin{algorithm2e}
\caption{DP-SGD in a Random Subspace}
\label{alg:opt_random_subspace}
{\bf Input:} 
Initial iterate $x^{(0)}$, 
dataset $\cD = \{s_j\}_{j \in [n]}$, 
per-step noise magnitude $\sigma$, 
number of updates $T$, 
learning rate $\eta$, 
and subspace dimension $r$. \\
Draw a random matrix of i.i.d. standard Gaussians $V \in \R^{d \times r}$  \\
Let $\widetilde{f}: \R^r \times \mathcal{S} \to \R$ be defined as 
    $\widetilde{f}(\zeta; s)  \defeq f(x^{(0)} + V \zeta ; s)$  \\
Run Algorithm~\ref{alg:noisy_SGD} based on the objective $\widetilde{f}$ but clip gradients by $O(\sqrt{r} (G_0 + \sum_{s=1}^{S_l} 2^{i/2} G_{2^{i-1}l} ) )$, initial iterate $\zeta^{(0)} = 0$, dataset $\cD = \{s_j\}_{j \in [n]}$, per-step noise magnitude $\sigma$, number of updates $T$, learning rate $\eta$, and Lipschitz constant $\widetilde{G} = \widetilde{G}_0$ of $\widetilde{f}$ (to be derived).
    Obtain output $\bar{\zeta}$. \\
{\bf Return:} $x^{(0)} + V \bar{\zeta}$.
\end{algorithm2e}

\subsection{Roadmap}
To simplify the analysis, we assume the dimension of subspace $r \in [d]$ is an even integer throughout, and thus, $r/2$ is also an integer.
Generalizing our results to odd $r$ is straightforward but tedious.
Conditioned on a random $V$, we define the following losses
\eqn{
    \widetilde{F}(\zeta ; \cD) \defeq
        F(x^{(0)} + V \zeta ; \cD), \quad
    \widetilde{f}(\zeta; s) \defeq 
        f(x^{(0)} + V\zeta ; s). 
}
We omit the dependence on the dataset for $\widetilde{F}$ and $F$ and assume they refer to the empirical loss unless otherwise mentioned.
The results to be presented require the following alternative assumption.
\begin{assumption}
\label{assm:subspace_extension}
The per-example loss $f(\cdot; s)$ is convex and restricted Lipschitz continuous with coefficients $\{G_k\}_{k = 0}^d$ for all $s \in \mathcal{S}$ for the same set of orthogonal projection matrices $\{P_k\}_{k=0}^d$.
\end{assumption}
The above assumption is stronger than merely letting the empirical loss be restricted Lipschitz continuous as in Assumption~\ref{assm:G_k}.
This condition will help us obtain tighter bounds on the Lipschitz constants of $\widetilde{F}$ and $\widetilde{f}$.
In the following, we first show two intermediate results hold with high probability over the random draw of $V$:
\begin{itemize}
    \item [(1)] There is a solution $\zeta$ that is a function of $V$ such that $ \widetilde{F}(\zeta) - \min_x F(x)$ is small and that 
        $\| \zeta \|_2$ is roughly $D / \sqrt{r}$ (up to a multiplicative factor), and
    \item [(2)] $\widetilde{f} (\cdot; s)$ is Lipschitz for all $s \in \cS$ with a coefficient that is roughly $\sqrt{r} G_0$ (up to a multiplicative factor).
\end{itemize}
To show both, we repeatedly exploit the technique adopted before: Split the ambient space into multiple orthogonal subspaces and bound the contribution of vectors projected onto each.
Fix $l = r / 2$. 
We define the following subspaces as before:
\begin{itemize}
\item $U_{0}=\range{P_l}$.
\item For $s=1,2,\cdots,\left\lfloor \log( d / l )\right\rfloor $, let $U_{s}\subset\range{P_{2^{s} l}}$
be a subspace with maximum dimension such that $U_{s}\perp U_{i}$
for all $i=0,\cdots,s-1$.
\item For $S_l =\left\lfloor \log( d/ l )\right\rfloor +1$, let $U_{S_l}\subset\R^{d}$
be the subspace such that $\oplus_{i=0}^{S_l}U_{i}=\R^{d}$ and $U_{S_l}\perp U_{i}$
for all $i=0,\cdots,S_l-1$. 
\end{itemize}
Finally, let $Q_{s}$ be the orthogonal projection onto the subspace $U_{s}$ for $s \in \{0, \dots, S_l]$.

\subsection{Part (1): Distance to Optimum and Diameter Bound}
\begin{lem}\label{lem:error_difference_and_diameter_bound}
Denote the first $l$ rows of $V$ by $V_l$. 
There exists a mapping $\zeta: \R^{ l \times r } \to \R^r$ such that
\[
 \normtwo{ \zeta( V_l ) } \lesssim D / \sqrt{r}
\]
with probability at least $1 - \exp(-\Omega(r) )$ over the random draw of $V_l$, and
\begin{align*}
    \widetilde{F}( \zeta( V_l ) ) =
    F( x^{(0)} + V \cdot \zeta( V_l  ) )
 \lesssim
    \min_{x} F(x) + \sum_{s=1}^{S_l} 2^{s/2} G_{2^{s-1} l}\cdot D
\end{align*}
with probability at least $1 - \exp(-\Omega(r) )$ over the random draw of $V$.
\end{lem}
While our work focuses on private learning, Lemma~\ref{lem:error_difference_and_diameter_bound} also presents connections to the concept of intrinsic dimension.
In particular, a simple corollary is that when gradients of the objective lie in a subspace of rank less than $l$, optimizing within a random subspace of dimension $r$ yields no extra loss with high probability.

\begin{proof}[Proof of Lemma~\ref{lem:error_difference_and_diameter_bound}]
Let $x^{*} \defeq \argmin_x F(x)$. 
We provide a constructive proof.
To simplify notation, we write $\zeta(V_l)$ as $\zeta$ when there's no ambiguity.
Without loss of generality, assume the range of $P_l$ is the set of vectors with possibly non-zero first $l$ coordinates and zeros for all remaining coordinates. 
Since $V_l V_l^{\top}$ is invertible almost surely,
we define $\zeta (V_l) \defeq V_l^{\top}(V_l V_l^{\top})^{-1}(x^{*}-x^{(0)})_{[l]}$, 
where $(x^{*}-x^{(0)})_{[l]} \in \R^l$ is the vector of the first $l$ coordinates of $x^{*}-x^{(0)}$.
Define the error vector
\begin{align*}
\epsilon & \defeq
    x^{(0)}+ V \zeta -x^{*}  =
    x^{(0)}-x^{*}+VV_l^{\top}(V_l V_l^{\top})^{-1}(x^{*}-x^{(0)})_{[l]}.
\end{align*}
By definition, $\epsilon_{i}=0$ for all $i\in[l]$.

We now bound the difference $F(x^{(0)}+V\zeta)-F(x^{*})$.
By the Mean Value Theorem, 
\[
F(x^{(0)}+V\zeta) = 
    F(x^{*}) + 
    \nabla F(\eta)^{\top}\epsilon
\]
for some $\eta$ that is a convex combination of $x^{(0)}+V\zeta$ and $x^{*}$. 
Now, we bound the error term
\begin{align*}
\nabla F(\eta)^{\top}\epsilon &=
    \sum_{s=1}^{S_l}(Q_{s}\nabla F(\eta))^{\top}(Q_{s}\epsilon) 
    \leq\sum_{s=1}^{S_l}\|Q_{s}\nabla F(\eta)\|_{2}\cdot\|Q_{s}\epsilon\|_{2},
\end{align*}
where we used the fact that $Q_0 \epsilon = 0$, since $\epsilon_i = 0$ for $i\in[l]$ and the assumption on the range of $P_l$.
For a fixed $s \in \{1, \dots, S_l \}$, since $V_{s}\perp\text{range}(P_{2^{s-1} l})$, 
\eqn{
    \|Q_{s}\nabla F(\eta)\|_{2}\leq G_{2^{s-1} l}.
}
We now bound $\|Q_{s}\epsilon\|_{2}$.
Since $l = r / 2$, standard results in random matrix theory~\cite[Corollary 5.35]{vershynin2010introduction} show that
\[
V_{l} V_{l}^{\top}\succeq\Omega(r)\cdot I_{l}, 
\]
with probability at least $1 - \exp(- \Omega(r) )$.\footnote{We used the one-sided version of \cite[Corollary 5.35]{vershynin2010introduction} which follows from Gaussian concentration.}
Hence, 
\[
\|\zeta \|_{2}^{2}=\|(x^{*}-x^{(0)})_{[l]}\|_{(V_lV_l^{\top})^{-1}}^{2} \lesssim
    \frac{1}{r}\|(x^{*}-x^{(0)})_{[l]}\|_{2}^{2}\leq\frac{D^{2}}{r}
\]
with probability at least $1 - \exp(- \Omega(r) )$.
Since $\epsilon_{i}=0$ for all $i\in[l]$, we can write $\epsilon= u +\sum_{i=1}^{r} \zeta_i v_i$, 
where $u \in \R^d$ and $v_i \in \R^d$ are defined as 
\eqn{
    u_j = 
    \begin{cases}
    0, & \quad j \le l \\
    (x^{(0)} - x^* )_j, & \quad \text{otherwise} \\
    \end{cases}, \quad
        (v_i)_j = 
    \begin{cases}
    0, & \quad j \le l \\
    V_{j, i}, & \quad \text{otherwise} \\
    \end{cases}.
}
For any fixed $i \in \{1, \dots, r\}$, $\zeta$ is independent of $v_i$ by definition, since $\zeta$ only depends on the first $l$ rows of $V$, whereas $v_i$ only depends on the last $(d - l)$ rows of $V$. 
Recall that $V_{j,i}$ is an independent standard Gaussian.
Thus, conditioned on $\zeta(V_l)$,
\eqn{
    &\bracks{ \sum_{i=1}^{r}\zeta_{i} v_i}_j = 0, \;\;  j \le l, \quad\\
    &\bracks{ \sum_{i=1}^{r}\zeta_{i} v_i}_j \sim 
    \cN \bracks{ 0,\|\zeta\|_2^2 }, \;\;  j  > l.
}
Recall that the range of $P_l$ is the set of vectors with possibly non-zero first $l$ coordinates and zeros for all remaining coordinates.
Since $Q_s$ is an orthogonal projection matrix, one has $Z = \frac{1}{\|\zeta\|_2^2} \|Q_s\sum_{i=1}^{r}\zeta_i v_i\|^2_2  \sim \chi^2_{r_s} $, where $r_s \leq \rank(Q_s)$.
We now show that conditioned on $\zeta(V_l)$, 
\begin{align}
    \label{eq:concentration_Z}
    \Pr\sbracks{ Z\geq 2^{s}l }\leq \exp(-\Omega(2^{s-1}r)).
\end{align}
Recall $2^sl\geq \rank(Q_s) \ge r_s$.
By standard concentration property of $\chi^2$-variables~\cite{laurent2000adaptive}, one has
\begin{align*}
    \Pr[Z -r_s\geq 2\sqrt{r_s t}+2t]\leq \exp(-t),
\end{align*}
for all $t \ge 0$.
Setting $t=\Theta(2^{s-1}r)$ yields~\eqref{eq:concentration_Z}.
Taking the union bound over $s \in \{1, \dots, S_l\}$, one has 
\begin{align*}
\Pr\Big[\|Q_s\sum_{i=1}^{r}\zeta_i v_i\|_2^2
\leq
    2^sl\cdot\|\zeta\|_2^2, \;\forall s\in[S_l]\Big] 
        \geq 1-\sum_{s=1}^{S_l}\exp(-\Omega(2^{s-1}r))\geq 1-\exp(-\Omega(r)).
\end{align*}
Recalling that $\normtwo{\zeta} \lesssim D / \sqrt{r}$ with probability at least $1 - \exp(-\Omega(r))$, we conclude that with probability at least $1 - \exp( -\Omega(r))$, one has
\eqn{
\nabla F(\eta)^{\top}\epsilon &\leq
    \sum_{s=1}^{S_l}\|Q_{s}\nabla F(\eta)\|_{2} \cdot\|Q_{s}\epsilon\|_{2} \lesssim
    \sum_{s=1}^{S_l} 2^{s/2}G_{2^{s-1} l}\cdot D.
}
This completes the proof.
\end{proof}

\subsection{Part (2): Lipschitz Constant}
\begin{lem}\label{lem:subspace_extension_lipschitz}
Under assumption~\ref{assm:subspace_extension},
with probability at least $1 - \exp(- \Omega(r) ) $ over the random draw of $V$, 
the function $\widetilde{f}(\cdot; s): \R^r \to \R$ is 
$O \bracks{ \sqrt{r} \bracks{ G_0 + \sum_{i=1}^{S_l} 2^{i/2} G_{2^{i-1} l } } }$-Lipschitz for all $s \in \mathcal{S}$.
Consequently, on the same event, the function $\widetilde{F}(\cdot; \cD): \R^r \to \R$ is also $O \bracks{ \sqrt{r} \bracks{ G_0 + \sum_{i=1}^{S_l} 2^{i/2} G_{2^{i-1} l } } }$-Lipschitz.
\end{lem}
\begin{proof}[Proof of Lemma \ref{lem:subspace_extension_lipschitz}]
Applying the decomposition trick, one has
\eqn{
    \nabla_\zeta \widetilde{f} (\zeta)
= 
    V^\top \nabla f (x^{(0)} + V \zeta)
= 
    V^\top g_\zeta
=
    \sum_{i=0}^{S_l} (V^\top Q_i) (Q_i g_\zeta). 
}
Noting that $\rank(Q_i)\leq 2^{i}l$, a non-asymptotic version of the Bai-Yin Theorem~\cite{vershynin2010introduction} shows that
\eqn{
    \| V^\top Q_i \|_\text{op} \lesssim \sqrt{ r + 2^{i}l},
}
with probability at least $1 - \exp\Big(- \Omega(r+2^{i}l)\Big)$ for each $i \in \{0, \dots, S_l\}$. 
One can see this by diagonalizing $Q_i$ and recalling that orthogonal projection matrices only have eigenvalues either $0$ or $1$. 
Finally, a simple application of the union bound shows that 
\eqn{
\|\nabla_\zeta \widetilde{f}(\zeta)\|_{2}
\leq 
    \sqrt{r} G_{0}+\sum_{i=1}^{S_l} \sqrt{r+ 2^il }\cdot G_{2^{i-1} l} 
\lesssim
    \sqrt{r} \bracks{
        G_{0} + \sum_{i=1}^{S_l} 2^{i / 2} G_{2^{i-1} l}
    },
}
with probability at least $1-\sum_{i=1}^{S_l}\exp\big(-\Omega(r+2^il) \big) \gtrsim 1 - \exp( - \Omega (r))$, where we used Assumption~\ref{assm:subspace_extension}.
This concludes the proof.
\end{proof}

\subsection{Bounds for Excess Empirical Loss}
We now put everything together and show that under certain conditions, with an appropriately chosen dimension, optimizing in a random subspace of such dimension yields excess risk bounds that are dimension-independent.
\begin{theorem}\label{thm:subspace_extension}
Let $\delta \in (0, \frac{1}{2}]$ and $\epsilon \in (0, 10]$. 
Under assumption~\ref{assm:subspace_extension}, set
$T=\Theta(n^2 + r \log^2 r)$,
$\sigma=\Theta \bracks{ \frac{\sqrt{T\log(1/\delta)}}{n\epsilon} }$, 
$\eta=\sqrt{\frac{ \widetilde{D}^2 }{T\cdot \widetilde{G}_{0}^{2} \cdot r \sigma^2 }}$,
and $\alpha=0$, 
where $\{\widetilde{G_k}\}_{k=0}^d$ denote the restricted Lipschitz coefficients of $\widetilde{F}(\cdot ; \cD)$, and $\widetilde{D}$ is the diameter bound of $\zeta(V_l)$, both of which are conditioned on $V$. 
DP-SGD in a random subspace (Algorithm~\ref{alg:opt_random_subspace}) is $(\epsilon,\delta)$-DP, and with probability at least $1 - \exp( -\Omega( r ) )$ over the draw of $V$,
\eqn{
    \E \sbracks{
        F( x^{(0)} + V \cdot \bar{\zeta} ) - \min_x F(x)
    } \lesssim
        \frac{ \bracks{ G_0 + K(l) } D \sqrt{ r \log (1/\delta) } }{ \epsilon n } + K(l) D ,
}
where the expectation is over the randomness of DP-SGD, and 
$K(l) = \sum_{s=1}^{S_l} 2^{s/2} G_{2^{s-1} l}$.

Moreover, if $G_k \le G_0 k^{-c}$ for each $k$ for some $c > 1/2$, and in addition $n > \epsilon^{-1} \sqrt{ \log (1 / \delta) }$, optimizing the above bound with respect to $r$ yields
\eqn{
    \E \sbracks{
        F( x^{(0)} + V \cdot \bar{\zeta} ) - \min_x F(x)
    } \lesssim
        G_0 D   \bracks{ \frac{\sqrt{\log (1 / \delta)}}{\epsilon n} }^{2c / (1 + 2c)}.
}
\end{theorem}
\begin{proof}[Proof of Theorem~\ref{thm:subspace_extension}]
The privacy guarantee again follows from Lemma~\ref{lm:privacy_guarantee}.
We now apply Theorem~\ref{thm:DPERM} to bound the excess empirical loss for optimizing $\widetilde{F}(\cdot ; \cD)$ using Lemmata~\ref{lem:error_difference_and_diameter_bound} and~\ref{lem:subspace_extension_lipschitz}. 
By setting $k$ in Theorem~\ref{thm:DPERM} to be $r$, one obtains
\eqn{
    \E \sbracks{
        \widetilde{F}( \bar{\zeta} ) - \widetilde{F}( \zeta(V_l) )
    } & \lesssim
        \frac{ \widetilde{G}_0 \widetilde{D} \sqrt{ r \log (1 / \delta) } }{ \epsilon n } \\
      & \lesssim
        \frac{ \bracks{G_0 + K(l) } D \sqrt{r \log (1 / \delta)} }{\epsilon n}, 
}
with probability at least $1 - \exp(-\Omega(r))$ over the random draw of $V$.
Moreover, with probability at least $ 1 - \exp(-\Omega( r ))$ over the random draw of $V$, 
\eqn{
    \widetilde{F}( \zeta(V_l) ) - \min_x F(x) \lesssim K(l) D.
}
Thus, applying the union bound, one has
\eqn{
    \E \sbracks{
        \widetilde{F}( \bar{\zeta} ) - \min_x F(x)
    }
    \lesssim
        \frac{  \bracks{ G_0 + K(l) } D \sqrt{ r \log (1/\delta) } }{ \epsilon n } + K(l) D,
}
with probability at least $1 - \exp(-\Omega(r))$. 

Moreover, suppose that $G_k \le G_0 k^{-c}$ for each $k$ for some $c > 1/2$. 
Then, $K(l) \lesssim l^{-c} G_0 \lesssim r^{-c} G_0 $. Thus, 
\eqn{
    \E \sbracks{
        \widetilde{F}( \bar{\zeta} ) - \min_x F(x)
    } \lesssim
        G_0 D  \bracks{  \frac{\sqrt{r \log (1/\delta)}}{\epsilon n} + r^{-c} },
}
with probability at least $1 - \exp(-\Omega(r))$. 
Letting 
\eqn{
    r = \min \left\{ 
        d,  
        \left\lceil \left( \frac{\epsilon n}{\sqrt{\log(1/\delta)}} \right)^{\frac{2}{1+2c}} \right\rceil
    \right\},
}
one has on the event
\eqn{
    \E \sbracks{
        \widetilde{F}( \bar{\zeta} ) - \min_x F(x)
    } \lesssim
        G_0 D  \bracks{ \frac{\sqrt{\log (1 / \delta)}}{\epsilon n} }^{2c / (1 + 2c)}.
}
\end{proof}



